Controlling field asymmetry in nanoscale gaps for second harmonic generation

Plasmonic dimer antennas create strong field enhancement by squeezing light into a nanoscale gap. These optical hotspots are highly attractive for boosting nonlinear processes, such as harmonic generation, photoelectron emission, and ultrafast electron transport. Alongside large field enhancement, such phenomena often require control over the field asymmetry in the hotspot, which is challenging considering the nanometer length scales. Here, by means of strongly enhanced second harmonic generation, we demonstrate unprecedented control over the field distribution in a hotspot by systematically introducing geometrical asymmetry to the antenna gap. We use focused helium ion beam milling of mono-crystalline gold to realize asymmetric-gap dimer antennas in which an ultra-sharp tip with 3 nm apex radius faces a flat counterpart, conserving the bonding antenna mode and the concomitant field enhancement at the fundamental frequency. By decreasing the tip opening angle, we are able to systematically increase both field enhancement and asymmetry, thus enhancing second harmonic radiation to the far-field, which is nearly completely suppressed for equivalent symmetric dimer antennas. Combining these findings with second harmonic radiation patterns as well as quantitative nonlinear simulations, we further obtain remarkably detailed insights into the mechanism of second harmonic generation at the nanoscale. Our results open new opportunities for the realization of novel nonlinear nanoscale systems, where the control over local field asymmetry in combination with large field enhancement is essential to create nonreciprocal functionalities.

==> Sections/section-Experiments.tex <==
\section{Experiments}
\subsection{Fabrication}
All antennas discussed in the main text are fabricated using a three-step milling method based on Ga-FIB and He-FIB milling. First, a Ga-ion beam with a current of $10\,$pA (acceleration voltage $V_a=30\,$kV) is used to define the coarse shape of the antenna centered in a ($4\times4$)$\,$\textmu m milled glass window to avoid unwanted reflections from the surrounding gold during optical measurements, see Fig.~\ref{fig:fabrication}a. Subsequently, the exact antenna shape is defined by a He-ion beam ($V_a=35\,$kV) with a current of $3.5\,$pA (Fig.~\ref{fig:fabrication}b). For milling the gap, we reduce the He-ion beam current down to $1.5\,$pA (Fig.~\ref{fig:fabrication}c) to achieve controlled gap sizes and gold tips with a minimal radius of curvature. 

\begin{figure*}[h]
	    \centering
        \includegraphics[width=.99\linewidth]{s_Figures/SI-Exp_Fig1_V2.png}
        \caption{\textbf{Helium ion microscope images illustrating the three-step milling approach based on Ga-/He-FIB.} Antenna after Ga-FIB \textbf{a,} first  \textbf{b,} and second  \textbf{c,} He-FIB step. Scale bars, $100\,$nm. The inset in \textbf{a} shows an overview of the antenna and the surrounding ($4\times4$)$\,$\textmu m glass window. Scale bar, $1\,$\textmu m.} 
\label{fig:fabrication}
\end{figure*}

\subsection{Optical setup for SHG measurements}
Fig.~\ref{fig:setup} shows a scheme of the optical setup used for recording SHG spectra and radiation patterns. Broadening of the $100\,$fs laser pulse due to dispersion is precompensated by a single-prism pulse compressor before the objective. Design details can be found in Ref.~\cite{akturk_extremely_2006}.
 To record radiation patterns, we place a 1000-mm Betrand lens in front of the spectrometer (at the position of the dashed line in Fig.~\ref{fig:setup}) and replace the spectrometer grating by a mirror.
 
\begin{figure*}[h]
	    \centering
        \includegraphics[width=.99\linewidth]{s_Figures/SI-Exp_Fig2_V1.pdf}
        \caption{\textbf{Scheme of the optical setup.} The beam of a Ti:Sa laser is focused onto the sample with a high NA objective (100×, NA = 1.45, Nikon). A pulse compressor after the laser output is used to precompensate dispersion. The SH scattered light is analyzed using a spectrometer equipped with an EMCCD (see Methods in main text for details about manufacturers).} 
\label{fig:setup}
\end{figure*}

\subsection{Linear properties}

In Fig.~\ref{fig:expWL} we show the single measurements of the angle-dependent SH power from Fig.~4 in the main text, including the information about the bonding mode resonance at the FF (circles correspond to asymmetric-gap, squares to symmetric-gap antennas, respectively). We compare the strength of the scattering amplitude at the resonance, $A_\text{scatt}(\lambda_\text{res})$, to the strength of the scattering amplitude at the excitation wavelength of $840\,$nm, $A_\text{scatt}(840\,\text{nm})$. To ensure comparability, we only take into account antennas where the resonance is equal or close to $840\,$nm, i.e.~$A_\text{scatt}(840\,\text{nm})/A_\text{scatt}(\lambda_\text{res}) > 0.9$. Within this range we do not observe any dependence of the SH signal on the resonance position.

\begin{figure*}[h]
	    \centering
        \includegraphics[width=.99\linewidth]{s_Figures/SI-Exp_Fig3_V4.pdf}
        \caption{\textbf{Analysis of the linear bonding mode resonance.} Raw data of the angle-dependent SH power shown in Fig.~4 in the main text. The color code indicates the deviation of the scattering amplitude at the antenna resonance, $A_\text{scatt}(\lambda_\text{res})$, from the scattering amplitude at $840\,$nm, $A_\text{scatt}(840\,\text{nm})$. Circles correspond to asymmetric-gap, squares to symmetric-gap antennas, respectively.} 
\label{fig:expWL}
\end{figure*}

\subsection{Antenna geometry} \label{subsection:antenna geometry}

\begin{figure*}[h]
	    \centering
        \includegraphics[width=.99\linewidth]{s_Figures/FigS4_V4.png}
        \caption{\textbf{Contour analysis of SEM images.} \textbf{a,}~SEM image of an exemplary asymmetric-gap antenna. The yellow square denotes the gap region which is analyzed. \textbf{b,}~Line profile taken in the middle of the gap. Gray region denotes contours considered for the analysis. \textbf{c,}~Exemplary contours marked with dotted black line \textbf{b}. Orange lines are fitted to the tip side to determine the opening angle. The green circle is fitted to the apex of the tip and is used to determine the radius of curvature. From the crossing of the angle bisector (dashed purple line) with the contours from the left and the right side, the gap size is determined. \textbf{d,}~Tip opening angle $\alpha$ (top), gap size $g$ (middle) and radius of curvature $r$ (bottom) depending on contour number for the contours shown in \textbf{c}. \textbf{e,}~Dependence of gap size $g$ (top two plots) and radius of curvature $r$ (bottom two plots) on the tip opening angle for all asymmetric-gap (red) and symmetric-gap (blue) antennas shown in Fig.~4 in the main text.} 
\label{fig:figS6}
\end{figure*}

The antenna geometry determines the strength of the linear response (field enhancement) and in turn the strength of SH sources. Therefore, a detailed analysis of the geometry is needed to properly model the SH response of the system. To this end we analyse SEM images to obtain lateral dimensions of the antenna (Fig.~\ref{fig:figS6}) and employ AFM measurements to retrieve information of the height of the gold antenna and the glass pedestal (Fig.~\ref{fig:figS7}). The lateral dimensions are most important in the gap region where the majority of the SH sources are generated (Fig.~\ref{fig:figS6}a). Two critical parameters which describe the gap region are the gap size $g$ and the radius of curvature of the tip $r$. To determine these parameters systematically we have performed a contour analysis, where we first take the line scan across the gap of the SEM image (Fig.~\ref{fig:figS6}b) and consider contours which are within the shaded region (contours too close to the top surface of antenna or substrate become discontinuous along the edge and are therefore disregarded). For each of the selected contours we fit the dashed orange lines to the tip side in order to determine the tip opening angle, as well as the green circle into the tip apex to obtain the radius of curvature (Fig.~\ref{fig:figS6}c). The gap size is determined from the distance of the points where the angle bisector (the purple dashed line) crosses the two contours (tip contour and straight edge contour). By doing so for each of the contours of interest, we obtain statistics of the different tip opening angles, gap sizes and radii of curvature for a single structure providing us with a tool to systematically determine the geometry of the gap region (Fig.~\ref{fig:figS6}d). Performing this for all of the structures under consideration we see that there is a tip opening angle dependent trend for gap size and radius of curvature which is different for the two types of antennas (Fig.~\ref{fig:figS6}e). The upper two rows in Fig.~\ref{fig:figS6}e denote the angle-dependent gap size for asymmetric-gap (red) and symmetric-gap (blue) structures. For different tip opening angles the gap size stays more or less constant with an average of $(8.1\pm0.9)\,$nm for asymmetric-gap and $(9.3\pm0.9)\,$nm for symmetric-gap antennas. On the other hand, in the bottom two rows of Fig.~\ref{fig:figS6} we can see that the radius of curvature is decreasing from approximately $8\,$nm to $3\,$nm as the tip opening angle is reduced from 80° to 20°. This significant decrease in radius of curvature has a strong influence on the SH signal and is therefore implemented into the numerical model using the linear fit as presented in Fig.~\ref{fig:figS6}e. 

\noindent The height of the antenna and pedestal do not play a critical role in the strength of the field enhancement in the gap, but still influence the spectral position of the bright mode at FF. We therefore also perform AFM topography measurements to retrieve information of the height of antenna and pedestal. In Fig.~\ref{fig:figS7}a and b we show an AFM topography of an exemplary antenna (no gap included) and the corresponding height profile, respectively. We obtain a total pedestal height of $50\,$nm originating from Ga- and He-FIB. We verify this result by He-milling simple rectangular patterns with increasing doses (see Fig.~\ref{fig:figS7}c), where we can see a linear trend between pedestal height and ion dose (typical dose used in the fabrication process corresponds to $1.1\,$C/cm²).   

\begin{figure*}[h]
	    \centering
        \includegraphics[width=.99\linewidth]{s_Figures/FigS5_V2.pdf}
        \caption{\textbf{AFM measurements.} \textbf{a,}~AFM topography of the antenna. \textbf{b,}~Height profile recorded at the line in \textbf{a}. The height of antenna relative to the substrate after Ga- and He-FIB milling is $50\,$nm. From optical measurements we know that the gold platelet height is $40\,$nm. This implies $10\,$nm pedestal height produced during Ga-FIB milling. Fine milling using helium ions introduces additional $40\,$nm pedestal height. \textbf{c,}~ He-FIB depth depending on the used dose for exemplary rectangular patterns milled into a glass window created with Ga-FIB. Dose is increased from 0.1 up to 1.5 C/cm² in steps of 0.2 C/cm².} 
\label{fig:figS7}
\end{figure*}

\newpage

\subsection{Evaluation of efficiency}

We evaluate the performance of our antennas similar to Ref.~\cite{celebrano_mode_2015}, see Table~\ref{tab:tabS1}. To calculate the emitted photons per second at the SH, we have to take into account losses of the optical setup. Transfer functions of the single components, namely microscope objective, beam splitter, shortpass filter, mirrors, confocal lens, spectrometer mirror, grating, and EMCCD, are taken from the respective manufacturer data. Majority of SH radiation is emitted into the substrate half-space and we therefore assume a collection efficiency of $100\,\%$ equivalent to Ref.~\cite{celebrano_mode_2015}. Thus, for a wavelength of $420\,$nm we arrive at a detection efficiency of 0.04 resulting in $9.9\times10^3$ emitted SH photons, evaluated for the asymmetric-gap antennas with $\alpha=25^\circ$ shown in Fig.~4 in the main text. Finally, for the maximum SH conversion efficiency we calculate $\gamma_\text{SH}=1.7\times10^{-10}$. We want to emphasize that this is the same order of magnitude of what has been achieved in Ref.~\cite{celebrano_mode_2015} ($\gamma_\text{SH}=5.1\times10^{-10}$), although we are working in the sub-$500\,$nm wavelength regime, where gold exhibits strong damping, and the antennas do not exhibit a second resonance at the SH frequency.

\begin{table}[h]
\caption{Efficiency calculation}
\centering
\scalebox{0.83}{
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|cccccccc|}
\hline
\multicolumn{1}{|c|}{\textbf{Parameter}}&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}laser\\ wavelength\\ $\lambda_\text{exc}$\end{tabular}}&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}laser\\ rep. rate\\ $f_\text{rep}$\end{tabular}}&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}laser\\ pulse length\\ $\tau$\end{tabular}}&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}laser\\ avg. power\\ $P_\text{avg}$\end{tabular}}& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}NA\\ objective\end{tabular}}&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}spot\\ diameter\\ $\delta$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}laser\\ peak power\\ $P_\text{peak}$\end{tabular} \\ \hline
\multicolumn{1}{|c|}{\textbf{Unit}} & \multicolumn{1}{c|}{nm} & \multicolumn{1}{c|}{MHz} & \multicolumn{1}{c|}{fs} & \multicolumn{1}{c|}{\textmu W} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\textmu m} & W \\ \hline
\multicolumn{1}{|c|}{\textbf{Formula}} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$1.22\lambda/\text{NA}$}& $P_\text{avg}/(f_\text{rep}\tau)$ \\ \hline
\multicolumn{1}{|c|}{\textbf{Value}} & \multicolumn{1}{c|}{840} & \multicolumn{1}{c|}{80} & \multicolumn{1}{c|}{100}  & \multicolumn{1}{c|}{15} & \multicolumn{1}{c|}{1.45} & \multicolumn{1}{c|}{0.707} & 1.9 \\ \hline
\multicolumn{8}{|c|}{\textbf{}} \\ \hline 
\multicolumn{1}{|c|}{\textbf{Parameter}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}em. SH photons\\ $N$\end{tabular}}  & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SH power\\ $P_\text{SH}$\end{tabular}}  & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SH peak power\\ $P_\text{SH, peak}$\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}max. SH conv.\\ efficiency\\ $\eta_\text{SH}$\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}peak nonlinear\\ coefficient $\gamma_\text{SH}$\end{tabular}} & \multicolumn{2}{c|}{\multirow{4}{*}{}} \\ \cline{1-6} \multicolumn{1}{|c|}{\textbf{Unit}} & \multicolumn{1}{c|}{cts/s} & \multicolumn{1}{c|}{W} & \multicolumn{1}{c|}{W} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{W$^{-1}$} & \multicolumn{2}{c|}{} \\ \cline{1-6}
\multicolumn{1}{|c|}{\textbf{Formula}} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{$N\cdot E_\text{ph}$} & \multicolumn{1}{c|}{$P_\text{SH}/(f_\text{rep}\tau)$} & \multicolumn{1}{c|}{$P_\text{SH} / P_\text{avg}$}  & \multicolumn{1}{c|}{$P_\text{SH, peak}/\left(P_\text{peak}\right)^2$}  & \multicolumn{2}{c|}{}  \\ \cline{1-6}
\multicolumn{1}{|c|}{\textbf{Value}} & \multicolumn{1}{c|}{$9.9\times 10^3$}  & \multicolumn{1}{c|}{$4.7\times10^{-15}$}  & \multicolumn{1}{c|}{$5.9\times10^{-10}$} & \multicolumn{1}{c|}{$3.1\times10^{-10}$}   & \multicolumn{1}{c|}{$1.7\times10^{-10}$} & \multicolumn{2}{c|}{} \\ \hline
\end{tabular}}
\label{tab:tabS1}
\end{table}



==> Sections/section-Numerical_simulations.tex <==
\section{Numerical simulations}
\subsection{Overview}

\noindent The FEM simulations discussed in the main text were performed using COMSOL Multiphysics® 6.0~\cite{hadoop}. We used the “Wave Optics Module” to solve Maxwell’s equations in the frequency domain for our system in a two step process. First, we analyze the linear response of the system, which is then used to calculate $\textbf{P}_\text{S}^{(2\omega)}$ according to Eq.~(2) in the main text. In the second step, we use this source to drive the system at SH. 

The first task is to find the geometry which exhibits a bonding mode resonance at $840\,$nm, the wavelength of the pump laser. For all scenarios under consideration, the antenna is placed on top of a glass substrate (see Fig.~\ref{fig:figS1}a). The simulation region, as in the exemplary case, is a sphere with radius of 600~nm, where the volume surrounding the antenna has a radius $r_{\text{sur}} = 400\,\text{nm}$. In addition, a perfectly matched layer (PML) with thickness $t_\text{PML} = 200\,\text{nm}$ is introduced to mimic an open and non-reflecting infinite domain.

\begin{figure*}[ht]
	    \centering
        \includegraphics[width=.99\linewidth]{s_Figures/FigS1_V7.pdf}
        \caption{\textbf{Geometry used for COMSOL simulations}. \textbf{a,}~Side view of the complete simulation volume. The gold antenna is situated on top of a glass pedestal above a glass substrate. \textbf{b,}~Side view zoom to the antenna area. $l_{\text{a}}$ is the length of the antenna, $h_{\text{a}}$ is the antenna height, $h_{\text{p}}$ is the height of the glass pedestal, $r_{\text{t}}$ is the radius of curvature of the antenna at the tip. \textbf{c,}~Top view of the antenna area. $l_{\text{t}}$ is the tip length, $\alpha$ is the tip opening angle, $r$ is the radius of curvature at the tip, $g$ is the gap size, $w_{\text{a}}$ is the width of the antenna, and $r_c$ is the radius of curvature of the antenna corners.} 
\label{fig:figS1}
\end{figure*}

Heights of the gold antenna and the pedestal on which it resides due to He-FIB milling into the substrate, as sketched in the side view in Fig.~\ref{fig:figS1}b, are obtained from atomic force microscopy (AFM) measurements. The height of the gold platelet used as starting material is retrieved by optical transmission measurements (as discussed in~\cite{grossmann2019nonclassical}). In a typical structure, the antenna height $h_{\text{a}}$ is $40\,$nm, while the pedestal, produced during He-FIB milling, has a height of $50\,$nm. Moreover, the lateral dimensions as shown in the top view in Fig.~\ref{fig:figS1}c, are extracted from SEM images. AFM and SEM analysis are discussed in more detail in section~\ref{subsection:antenna geometry}. In all cases, antennas have been designed to have a width $w_{\text{a}}$ of $60\,$nm and a tip length $l_{\text{t}}$ of $30\,$nm, while the radius of curvature of the antenna corners $r_c$ is kept constant at $8\,$nm and radius of curvature at the tip $r_\text{t}$ at $3\,$nm. The tip opening angle $\alpha$ has been varied from 20° to 80°. The radius of curvature of the tip $r$ has been adapted for each structure, where smaller angles lead to sharper tips. Moreover, changes of the tip opening angle lead to changes in the coupling strength between two antenna arms. Therefore, the length of the antenna rods has been adapted for each tip opening angle to re-adjust the bonding mode resonance to $840\,$nm. 


\subsection{Linear simulations}

\noindent The linear response of the system, that is the scattering spectrum and the near-field response, are simulated using the scattered field formulation implemented in COMSOL. Since the size of the collimated beam that is used for excitation in the white-light scattering experiment is approximately $2\,$\textmu m, we use a plane wave propagating in $+z$ direction, polarized along the long axis of the antenna as excitation source (background field). Due to the presence of the glass-air interface the background field is calculated from s-polarized Fresnel coefficients for the glass and the air half-space separately. The excitation wavelength  ranges from 400 to $1000\,$nm and is discretized in steps of $10\,$nm.  The refractive index of glass is modeled using Sellmeier coefficients for borosilicate crown glass~\cite{Schott}, while the permittivity of gold is modeled using single-crystal experimental data by Olmon et al.~\cite{Olmon}, as it has been demonstrated to accurately represent the optical response of our gold microplatelets (see~\cite{grossmann2019nonclassical}).

\begin{figure*}[ht]
	    \centering
        \includegraphics[width=.99\linewidth]{s_Figures/FigS2_V14.pdf}
        \caption{\textbf{Linear spectra}. Scattering cross sections of asymmetric-gap \textbf{a,}~and symmetric-gap \textbf{b,}~antennas for different tip opening angles from 20° to 80°. All geometries were optimized such that the peak of the fundamental bonding mode resonance is at $840\,$nm.} 
\label{fig:figS2}
\end{figure*}

Scattering cross sections are presented in Fig.~\ref{fig:figS2}a,b for symmetric-gap and asymmetric-gap antennas, respectively. The geometry of each antenna is optimized to bring the bonding mode resonance to $840\,$nm by changing $l_{\text{a}}$. The small peak at $600\,$nm corresponds to the antibonding resonance as verified by inspection of its mode pattern. All of the structures show only weak response at $420\,$nm, corresponding to the SH wavelength, providing us with the possibility to test how symmetry breaking influences SHG without major influence by antenna-enhanced radiation effects. 

Using Eq.~(4) from the main text we can calculate the expectation for the SH signal considering only the field at FF. From such simple considerations it is expected to observe no SHG from symmetric-gap antennas, while in the case of asymmetric-gap antennas SHG can be tuned by a factor of 30 by changing the tip opening angle from 80° to 20° (see Fig.~\ref{fig:figS2_1}).

\begin{figure*}[ht]
	    \centering
        \includegraphics[width=.99\linewidth]{s_Figures/FigS2_1_V1.pdf}
        \caption{\textbf{SHG expectation from linear simulations}. Radiated SH power depending on the tip opening angle as expected from linear simulations.} 
\label{fig:figS2_1}
\end{figure*}



\subsection{Nonlinear simulations}

\noindent As discussed in the main text, the second order nonlinearity of gold nanoantennas originates from breaking the centrosymmetry of the gold crystal lattice at the surface of the structure, with $\chi^{(2)}_{\text{S},\perp,\perp,\perp}$ being the dominant term of the $\rttensortwo{\chi}^{(2)}_\text{S}$ tensor. Other nonlinear components, such as $\chi^{(2)}_{\text{S},\parallel,\perp,\perp}$ as well as bulk contribution (values taken from Ref.~\cite{wang2009surface}), have been tested and show no significant influence on the SH response of our system. Due to the discontinuity of the electric field normal component at the surface, a controversy existed regarding whether the inside or the outside field at FF should be taken to evaluate the SH response, which was resolved by Sipe et al.~\cite{sipe1980analysis}. They have demonstrated that in order to accurately model SH from metal surfaces, the FF fields from inside the metal should be utilized and generated SH sources should be placed just outside of the metal. 

%Therefore, second harmonic polarization can be expressed as:

%\begin{equation}
%     \label{SH polarization}
%     \textit{\textbf{P}}_{s}^{(2\omega)}(\textit{\textbf{r}})=\varepsilon_{0}\chi^{(2)}_{s,\perp,\perp,\perp}E_{\perp}^{(\omega)}E_{\perp}^{(\omega)}\hat{r}_{\perp}\delta(\textit{\textbf{r}}-\textit{\textbf{r}}_{s}),
% \end{equation}

% \noindent where $\textit{\textbf{r}}_{s}$ is a position vector pointing at the surface, and $\chi^{(2)}_{S,\perp,\perp,\perp}$ is the most dominant component of second order susceptibility tensor describing a process in which two perpendicular components of electric field at fundamental frequency (FF) are combined to produce second harmonic polarization current $j_{s}=\partial_{t}P_{s}^{(2\omega)}$ oscillating  perpendicular to the surface. 

There are several approaches to include surface sources into Maxwell's equations, and subsequently to couple them to a numerical solver. One of the possibilities has been explored by Reddy et al.~\cite{reddy2017revisiting}, who introduced polarization sources at the interface via modified boundary conditions. The new boundary condition for the tangential component of the electric field $\textbf{E}_{\parallel}$, in the presence of the current oscillating perpendicular to the surface, reads as

\begin{equation}
    \label{Reddy}
    \Delta{\textbf{E}}_{\parallel}^{(2\omega)}=-\frac{1}{\varepsilon'}\nabla_{\parallel}P_{\text{S},\perp}^{(2\omega)}(\textbf{r}_\text{S}),
\end{equation}

\noindent where $\nabla_{\parallel}$ is the tangential component of the vector derivative, $P_{\text{S},\perp}^{(2\omega)}$ is the perpendicular component of the SH polarization source and $\varepsilon'$ is the permittivity of the surrounding medium at SH. One of the limitations of this method becomes obvious when considering structures which do not have a smooth surface (as in our case), yielding an undefined vector derivative $\nabla_{\parallel}$. 
We have also considered the auxiliary field method introduced by Yang et al. within their framework for general electromagnetism at the nanoscale~\cite{yang2019general}. With this approach, it is possible to circumvent the need for calculating vector derivatives tangential to the surface, rendering the method more robust. However, by introducing auxiliary fields, simulation time is prolonged as it requires the use of more stable non-iterative solvers. Finally, we have implemented SH sources directly by stating them in the weak form as it was shown by Yang and Ciracì~\cite{yang2022second}.  We present a simple derivation of the weak form starting from Maxwell's wave equation for the electric field 

\begin{equation}
    \label{Weak form 1}
    \nabla \times \frac{1}{\mu}\nabla \times \textbf{E}-\frac{\omega^2}{c^2}\varepsilon \textbf{E}=-i\omega\mu_{0}\textbf{j}.
\end{equation}

\noindent Here we adopt the engineering $+i\omega t$ convention as it is used in COMSOL, yielding a negative sign for the current term. If we consider an arbitrary current source oscillating perpendicular to the surface $\textbf{j}=j_\text{S}\hat{r}_{\perp}\delta(\textbf{r}-\textbf{r}_\text{S})$, where $j_\text{S}$ can be expressed via polarization $P_\text{S}$, i.e. $j_\text{S}= \partial_{t} P_\text{S}$, then by multiplying this expression with the test field $\Tilde{\textbf{E}}$ and integrating over the whole volume we obtain

\begin{equation}
    \label{Weak form 2}
    \int_{V} dV \bigg[ \nabla \times \frac{1}{\mu}\nabla \times \textbf{E}-\frac{\omega^2}{c^2}\varepsilon \textbf{E}\bigg]\cdot\Tilde{\textbf{E}} =\omega^2\mu_{0}\int_{V}dV \textbf{P}_\text{S}\cdot\Tilde{\textbf{E}}.
\end{equation}

\noindent The volume integral on the right side collapses to a surface integral yielding a surface contribution in the weak form

\begin{equation}
    \omega^2\mu_{0}\int_{S}dS P_{\text{S},\perp}\Tilde{E}_{\perp}.
\end{equation}

To put the methods to test, we have inspected the influence of the shape of the sharp edges on the SH radiation patterns. The results provided by the weak form are independent of small changes in the geometry of the structure close to sharp edges which is not the case for the boundary condition method. Therefore, from the considered methods the weak form method provides the most robust and economical way to simulate SH response. 


\subsection{Influence of $\chi^{(2)}$ on radiation patterns}

\noindent One of the main uncertainties when it comes to modeling the nonlinear response of antennas, is the uncertainty in the experimentally obtained numerical values of $\chi^{(2)}_{\text{S},\perp,\perp,\perp}$ (shorthand notation $\chi^{(2)}$) for different interfaces. In this section we therefore analyze the influence of $\chi^{(2)}$ on radiation pattern and radiated power of the system under investigation. 

As a starting point we perform nonlinear simulations by choosing the experimentally obtained $\chi^{(2)}_{a}=6.5\cdot10^{-18}\mathrm{m^{2}/V}$ value measured by Wang et al.~\cite{wang2009surface}, which has been determined for a gold-air interface. It is common practice to use the same value of the parameter on the other interfaces as well~\cite{o2015predicting}, in our case the gold-glass interface. Using this simplification we calculate radiation patterns of our antenna structures using the far-field expansion Matlab toolbox RETOP 8.1~\cite{yang2016near}. The second row of Fig.~\ref{fig:figS3} shows that the radiation patterns for the short axis of the asymmetric-gap antenna and both radiation patterns of the symmetric-gap antenna do not fit to the corresponding experimental data displayed in the first row of the figure. To resolve this evident discrepancy we have tested theoretically calculated $\chi^{(2)}$ parameters which depend on the dielectric material neighboring the gold interface~\cite{benedetti2010engineering,vincenti2012gain}. Implementing the formula for $\chi^{(2)}$ given in this publication yields for the gold-air interface $\chi^{(2)}_{a}=(3.8-i0.5)\cdot10^{-18}\mathrm{m^{2}/V}$ and $\chi^{(2)}_{g}=(-0.8+i0.1)\cdot10^{-18}\mathrm{m^{2}/V}$ for the gold-glass interface, respectively. However, this choice of $\chi^{(2)}$ values does not yield a better match between simulations and experiment as it can be seen by inspecting the bottom row in Fig.~\ref{fig:figS3}. 

\begin{figure*}[ht]
	    \centering
        \includegraphics[width=.99\linewidth]{s_Figures/FigS3_V3.pdf}
        \caption{\textbf{Radiation patterns for $\chi^{(2)}$ values taken from the literature.} For comparison, the first row displays the measured radiation patterns also shown in Fig.~3 in the main text. In the second row radiation patterns are plotted using the experimentally determined value of $\chi^{(2)}$ according to Ref.~\cite{wang2009surface}. In the third row, $\chi^{(2)}$ values for two interfaces have been calculated using a formula derived in Refs.~\cite{benedetti2010engineering,vincenti2012gain}.} 
\label{fig:figS3}
\end{figure*}

Due to this uncertainty it seems to be appropriate to use $\chi^{(2)}$ as a fitting parameter. Note that the general formula for the response of the system upon driving it with the source $\textbf{P}_\text{S}$ is linear. According to~\cite{novotny2012principles} the electric field at any position $\textbf{r}$ can be calculated from the following expression 

\begin{equation}
    \label{chi 1}
    \textbf{E}(\textbf{r})=\frac{\omega^2\mu}{\varepsilon_{0}c^2}\int_{V_{0}}{\overleftrightarrow{\textbf{G}}_{tot}(\textbf{r},\textbf{r}_{0})\textbf{P}_\text{S}(\textbf{r}_{0})dr_{0}^3}.
\end{equation}

\noindent Here, $\mu$ is the relative permeability of the surrounding medium and $\overleftrightarrow{\textbf{G}}_{tot}(\textbf{r},\textbf{r}_{0})$ is a dyadic Green's function, representing the response of the system at position $\textbf{r}$ upon point source excitation at position $\textbf{r}_{0}$. The integration is performed over the antenna volume $V_{0}$. In the case of a homogeneous interface, a change in $\chi^{(2)}$ does not affect the resulting radiation pattern  $p(\textbf{r})\propto\left| \textbf{E}(\textbf{r})\right|^2$, and only influences the total radiated power \mbox{$P_\text{SH}=\int p(\textbf{r})d\Omega$}. 
However, since our system has two interfaces with different non-negligible SH source contributions -- gold-glass and gold-air interface -- we have to split the integral and consider a correct scaling of both $\chi^{(2)}$ parameters. Therefore, we state Eq.~\eqref{chi 1} in the following form 

\begin{equation}
    \label{Chi2 2}
    \textbf{E}(\textbf{r})=s_{a}\textbf{E}_{a0}(\textbf{r})+s_{g}\textbf{E}_{g0}(\textbf{r}),
\end{equation}

\noindent where $s_{a}$ and $s_{g}$ are scaling factors for the respective $\chi^{(2)}$ parameters, such that $\chi^{(2)}_{a}=s_{a}\chi^{(2)}_{a0}$, $\chi^{(2)}_{g}=s_{g}\chi^{(2)}_{g0}$. $\textbf{E}_{a0}(\textbf{r})$ and $\textbf{E}_{g0}(\textbf{r})$ are fields radiated by the antenna, driven only by sources at the respective interfaces, where in both cases we apply the normalization $\chi^{(2)}=1\,$m²/V. Taking the absolute square of the total field yields

\begin{equation}
    \label{Chi2 3}
    \left| \textbf{E}(\textbf{r})\right|^2=\left|s_{a}\right|^2\bigg\{\left|\textbf{E}_{a0}(\textbf{r})\right|^2+\left|\frac{s_{g}}{s_{a}}\right|^2\left|\textbf{E}_{g0}(\textbf{r})\right|^2+2\left|\frac{s_{g}}{s_{a}}\right|\left|\textbf{E}_{g0}(\textbf{r})\right|\left|\textbf{E}_{a0}(\textbf{r})\right|\text{cos}(\Delta\phi_0+\Delta\phi_{s})\bigg\},
\end{equation}

\noindent
where $\Delta\phi_0=\phi_{g0}-\phi_{a0}$ is the phase difference for the case of $s_{a}=s_{g}=1$, while $\Delta\phi_s=\phi_{g}-\phi_{a}$ is the phase difference due to scaling. We can see that the shape of the radiation pattern depends on the relative size of the $\chi^{(2)}$ parameters -- since they are complex-valued numbers, radiation patterns depend on the relative magnitudes and phase differences of the two nonlinear susceptibilities. Therefore, we keep one of the two parameters constant and scale the other. We choose to fix $s_{a}=1$ and scale $s_{g}$ (from here on referred to as $s$) in the complex plane, that is we scale the gold-glass susceptibility relative to the gold-air susceptibility $\chi^{(2)}_{g}=s\cdot \chi^{(2)}_{a}$. 

\begin{figure*}[ht]
	    \centering
        \includegraphics[width=.99\linewidth]{s_Figures/FigS4_V8.pdf}
        \caption{\textbf{Finding the optimal $s$ parameter}. \textbf{a,}~Complex plane plot. Locations of optimal radiation patterns are denoted with red x markers, on top of the color plot showing the dependence of the logarithm of total distance $d$ between experiment and simulation (power curves) on the scaling parameter $s$ (position in the complex plane). The optimum of the scaling parameter is marked by a white x. \textbf{b,}~Normalized SH power depending on the tip opening angle $\alpha$ for simulation (solid line) and experiment (scattered data) for asymmetric-gap (red) and symmetric-gap (blue) antennas. For each of the experimental data points, the distance is calculated from the corresponding simulated curve. The total distance $d$ is the sum of individual distances $d_{i}$ and serves as a minimization parameter for fitting. \textbf{c,}~Simulated curves are scaled with factor $\sigma$ due to uncertainty in the experimentally obtained data. The minimum in distance is obtained for a scaling factor of 0.9.} 
\label{fig:figS4}
\end{figure*}

To match the experimental data with simulations, we considered both types of experimental results presented in the main text: radiation patterns for a fixed angle (40° -- see Fig.~3 in the main text) and SH power depending on the tip opening angle (Fig.~4 in the main text). In a first step we calculate radiation patterns for a limited region in the complex plane for amplitudes $\left|s\right|$ between 0 and 2 in steps of 0.1 and phase $\phi_{s}$ between 0 and $2\pi$ in steps of 10°. Radiation patterns and the corresponding radiated power are calculated by superimposing the scaled far fields emitted by the antenna, independently driven with nonlinear sources at two interfaces (see Eq.~\eqref{Chi2 2}).

Examining the radiation patterns at different regions of the complex $s$ plane (as in the main text Fig.~3b,c), it becomes obvious that only radiation patterns simulated for values of $s$ in a small part of the first quadrant resemble the experimentally observed ones, i.e.~having a characteristic asymmetry along the short axis of the asymmetric-gap antenna (see Fig.~3b,d main text). By analyzing the detailed shape of the radiation patterns as well as the relative magnitudes of the intensities of long and short axis patterns for both asymmetric-gap and symmetric-gap antenna, one can single out the best fitting patterns for a limited set of points in the complex plane, the position of these points are denoted with red x's in Fig.~\ref{fig:figS4}a.

This set of optimal values for scaling parameters $S=\{s_{1},s_{2},...\}$ is now used as a set of possible values for fitting of the power curves which is done as shown in Fig.~\ref{fig:figS4}b. Distances $d_{Si},d_{Ai}$ (where distance is defined as $d=\left|P_\text{SH,e}-P_\text{SH,s}\right|$, indices e and s denote experiment and simulation, respectively) between experimentally obtained normalized SH signals and corresponding simulated ones, for both asymmetric-gap (index A) and symmetric-gap (index S) antenna, are retrieved and summed up, yielding a total distance $d=\sum(d_{Ai}+d_{Si})$. The distance is minimized to retrieve an optimal value for the scaling parameter $s$. Since both experimental and simulated data are normalized to the equivalent reference SH signal (symmetric 80°) and due to uncertainty in the experimental result, we introduce a scaling factor $\sigma$ for the simulated curves. We can see in Fig.~\ref{fig:figS4}c that the minimum in distance between experiment and simulation, depending on the scaling factor $\sigma$, is reached for a value $\sigma=0.9$. There, the optimal scaling parameter $s$ for fitting both radiation patterns as well as SH power as a function of the tip opening angle data, has a value of 0.55 in amplitude and a phase of 50$^{\circ}$ ($= 5/18\pi$ radians).

\subsection{Semi-analytical calculation of radiation patterns - effective dipole model}

\noindent In this section we demonstrate how the radiation pattern of an arbitrary radiating system placed above a planar interface can be calculated by employing a semi-analytical approach (similar to~\cite{bouhelier2003near}). Two main ingredients have to be considered, namely the total near-field polarization $\textbf{P}(\textbf{r}_{0})$ (in the text below it will be referred to as “source”), and far-field Green's tensor of a point dipole $\overleftrightarrow{\textbf{G}}(\textbf{r},\textbf{r}_{0})$ for the geometry under consideration (here a planar interface between two half spaces). Here, $\textbf{r}_{0}=(x_{0},y_{0},z_{0})$ is position of a point source located above the planar interface, while the field is evaluated at a far-zone point $\textbf{r}=(x,y,z)$.
The electric field in the far-field $\textbf{E}(\textbf{r})$ can be calculated using Eq.~\eqref{chi 1}, where the total polarization $\textbf{P}(\textbf{r}_{0})$ is used instead of a nonlinear source polarization $\textbf{P}_\text{S}(\textbf{r}_{0})$.

We separate the Green's tensor into a part which solely depends on the position in the far-field and a scalar function $\textit{f}(\textbf{r},\textbf{r}_{0})$ which carries information of the position of the source in the near-field $\overleftrightarrow{\textbf{G}}(\textbf{r},\textbf{r}_{0})=f(\textbf{r},\textbf{r}_{0})\overleftrightarrow{\textbf{G}}(\textbf{r})$. This allows us to take the tensor out of the integral and to simplify the calculation. The scalar function $f$ is defined as

\begin{equation}
    \label{Effective-dipole far field 2}
    f(\textbf{r},\textbf{r}_0)=\text{exp}\left[-ik_1\left(x_0\frac{x}{r}+y_0\frac{y}{r}-z_0\sqrt{1-\left(\frac{n_2}{n_1}\frac{\rho}{r}\right)^2}\right)\right],
\end{equation}

\noindent where $k_{1}$ is a wavevector in the upper half-space, while $n_{1}$, $n_{2}$ are refractive indices of the upper and lower half-space, respectively.

The integration in Eq.~\eqref{chi 1} is performed over the volume $V_{0}$ of the radiating system. In the most general case one can perform the integration and calculate the radiation pattern, however, at the cost of losing the physical picture behind the process. Since our source is mostly localized within the tip and in order to resolve the aforementioned problem, we can perform a Taylor expansion of the scalar function $f$ and analyze the contribution from each term separately -- the expansion is performed around the center of mass of polarization $\textbf{r}_\text{cm}$ to minimize the error in the first term

\begin{equation}
    \label{Effective-dipole far field 3}
    f(\textbf{r},\textbf{r}_0)=f(\textbf{r},\textbf{r}_\text{cm})+\Delta \textbf{r}_0^\mathsf{T}\nabla f(\textbf{r},\textbf{r}_\text{cm})+\frac{1}{2}\Delta \textbf{r}_0^\mathsf{T} \left[\nabla\nabla^\mathsf{T}f(\textbf{r},\textbf{r}_\text{cm})\right]\Delta \textbf{r}_0+...\,.
\end{equation}

Moreover, due to the form of the function $\textit{f}$, none of the derivatives depend on the position in the near-field and can be taken out of the integral. Finally, the electric far-field can be calculated from the following expression:

\begin{align}
\label{Effective-dipole far field 4}
\begin{split}
\textbf{E}(\textbf{r})=\frac{\omega^2\mu_1}{\varepsilon_0c^2}\overleftrightarrow{\textbf{G}}(\textbf{r}) \sum_i \Bigl\{ & f(\textbf{r},\textbf{r}_{cm})\int_{V_{0}} \textbf{P}_i(\textbf{r}_0) dr_0^3 \\ & + \sum_j  \partial_jf(\textbf{r},\textbf{r}_{cm}) \int_{V_0} \Delta r_{0j}  \textbf{P}_i(\textbf{r}_0) dr_0^3\\ & + \frac{1}{2}\sum_{j,k} \partial_{jk}f(\textbf{r},\textbf{r}_{cm}) \int_{V_0} \Delta r_{0j} \Delta r_{0k} \textbf{P}_i(\textbf{r}_0) dr_0^3\\ & + ...\Bigr\},
\end{split}
\end{align}

\noindent where $\mu_1$ denotes the relative permeability of the upper half-space medium and summations $i, j, k$ run over the Cartesian components $x, y, z$. The first integral has only one term per component and is named effective dipole of a system. The second integral has three terms per component and corresponds to an effective quadrupole. The third integral has nine terms per component and is a measure of an octupole contribution of a system, and so on.

Due to symmetry of our structure and the excitation, an asymmetric-gap antenna will exhibit a strong effective dipole with zero $y$-component and non-zero $x$- and $z$-components. Moreover, since the effective dipole is the dominant term, shape and symmetry of the radiation pattern are already accurately represented by the first term of the Taylor expansion without the need of considering higher-order corrections, as shown in Fig.~\ref{fig:figS5}a. Nevertheless, by introducing both effective dipole and effective quadrupole (Fig.~\ref{fig:figS5}b), or even contributions up to the effective octupole (Fig.~\ref{fig:figS5}c), the obtained radiation patterns quickly converge to the full radiation patterns calculated with the Matlab toolbox (Fig.~\ref{fig:figS5}d). 

In the case of symmetric-gap antennas, the effective dipole will, due to symmetry reasons, solely have a non-vanishing $z$-component, yielding a circular radiation pattern with intensity mostly localized around the critical angle. However, the symmetric-gap antenna exhibits rather strong, out-of-phase $x$-polarization in the two antenna arms. Therefore, the expectation is that non-negligible $x$-quadrupole terms should be obtained which implies spreading of the radiation pattern lobes in the $x$-direction (Fig.~\ref{fig:figS5}b). Other, higher-order contributions hardly affect the shape of the radiation pattern (Fig.~\ref{fig:figS5}c). 


\begin{figure*}[h]
	    \centering
        \includegraphics[width=.99\linewidth]{s_Figures/FigS5_V5.pdf}
        \caption{\textbf{Semi-analytical calculation of radiation patterns}. Calculations for asymmetric-gap (two left columns) and symmetric-gap antenna (two right columns). \textbf{a}-\textbf{c,}~Calculations are performed using the semi-analytical approach  considering one, two and three orders of Eq.~\eqref{Effective-dipole far field 4}, respectively. \textbf{d,}~Radiation patterns calculated using Matlab toolbox (RETOP 8.1), which is equivalent to summing all the terms of the semi-analytical approach.} 
\label{fig:figS5}
\end{figure*}
